Learning the Distribution Map in Reverse Causal Performative Prediction

In numerous predictive scenarios, the predictive model affects the sampling distribution; for example, job applicants often meticulously craft their resumes to navigate through a screening systems. Such shifts in distribution are particularly prevalent in the realm of social computing, yet, the strategies to learn these shifts from data remain remarkably limited. Inspired by a microeconomic model that adeptly characterizes agents' behavior within labor markets, we introduce a novel approach to learn the distribution shift. Our method is predicated on a reverse causal model, wherein the predictive model instigates a distribution shift exclusively through a finite set of agents' actions. Within this framework, we employ a microfoundation model for the agents' actions and develop a statistically justified methodology to learn the distribution shift map, which we demonstrate to be effective in minimizing the performative prediction risk.

==> YK-macros.tex <==
\usepackage{bbm}
\def\Avar{\mathrm{Avar}}
\def\abs#1{\left|#1\right|}
\def\aff{\mathrm{aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{\mathrm{avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\DeclareMathOperator{\Tr}{Tr}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{\mathrm{bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}
\def\d{\mathrm{d}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{\mathrm{Ber}}
\def\bin{\mathrm{bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{\mathrm{cat}}
\def\Cov{\mathrm{Cov}}
\def\cov{\mathrm{cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{\mathrm{cl}}
\def\complex{{\bbC}}
\def\cone{\mathrm{cone}}
\def\conv{\mathrm{conv}}
\def\deq{\overset{d}{=}}
\def\det{\mathrm{det}}
\def\diag{\mathrm{diag}}
\def\diam{\mathrm{diam}}
\def\dist{\mathrm{dist}}
\def\dom{\mathrm{dom}}
\def\doop{\mathrm{do}}
\def\dto{\overset\mathrm{d}{\to}}
\def\Ex{{\bbE}}
\def\Exp{\mathrm{Exp}}
\def\exp{\mathrm{exp}}
\def\eg{{\it e.g.}}
\def\epi{\mathrm{epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\iid{\mathrm{iid}}
\def\ind{\perp \!\!\! \perp}
\def\intr{\mathrm{int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{\mathrm{KL}}
\def\ker{\mathrm{ker}}
\def\lspan{\mathrm{span}}
\def\maximize{\mathrm{maximize}}
\def\med{\mathrm{med}}
\def\minimize{\mathrm{minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\base{\mathrm{base}}
\def\ss{\mathrm{ss}}
\def\Poi{\mathrm{Poi}}
\def\Pr{{\bbP}}
\def\PU{{\mathrm{PU}}}
\def\peq{\overset\mathrm{p}{=}}
\def\plim{\mathrm{plim}}
\def\proj{\mathrm{proj}}
\def\prox{\mathrm{prox}}
\def\pto{\overset\mathrm{p}{\to}}
\def\ran{\mathrm{ran}}
\def\rank{\mathrm{rank}}
\def\reals{{\bbR}}
\def\relint{\mathrm{relint}}
\def\sign{\mathrm{sign}}
\def\supp{\mathrm{supp}}
\def\symm{{\bbS}}

\def\st{\textrm{subject to}}
\def\tr{\mathrm{tr}}
\def\tube{\mathrm{tube}}
\def\TV{\mathrm{TV}}
\def\unif{\mathrm{unif}}
\def\Var{\mathrm{Var}}
\def\var{\mathrm{var}}
\def\vct{\mathrm{vec}}
\def\veps{\varepsilon}
\def\vol{\mathrm{vol}}
\def\zeros{\mathbf{0}}
\def\ante{{\mathrm{ex-ante}}}
\def\PR{{\mathrm{PR}}}

\def\iid{{\sf i.i.d.}}
\def\indicator{\mathbbm{I}}
\def\sB{\operatorname{B}}
\def\sA{\operatorname{A}}
\def\sF{\operatorname{F}}

==> YK-thm-macros.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{result}[theorem]{Result}


==> section/reg_analysis.tex <==
\section{Regret Analysis on performative risk}\label{sec:Regret}
In this section, we demonstrate that the ``plug-in'' approach of learning the distribution map and plugging it into a performative prediction algorithm that requires knowledge of the distribution map, is often statistically more efficient than zeroth-order methods that avoid learning the distribution map and directly optimizes the performative risk. The plug-in approach also confers more practical advantages. If the learner wishes to enforce certain constraints (\eg\ to enforce fairness after the agents adapt \citep{maity2021Does,somerstep2023Learning}), then the plug-in approach can be readily adapted to such constrained performative risk minimization problems \citep{cotter2018Training,cotter2019Optimization}. On the other hand, adapting zeroth-order methods that avoid learning the distribution map to such constrained performative risk minimization problems seems non-trivial.

The learner's goal is to deploy models that are eventually close to the \textit{performative optimum} (not necessarily unique) $\theta^{\star} \in \argmin_{\theta}\PR(\theta)$, where $\PR(\theta)= \sum\nolimits_{a \in \cA} \cD_\theta(a)\Ex\big[\ell(\theta;Z)\mid A = a\big]$ as defined in \eqref{eq:PR-discrete-actions} and $\cA = \{0,1\}$. Then, to learn $\theta^{\star}$ we first learn $\cD_\theta(0)$ (and then $\cD_\theta(1)= 1-\cD_\theta(0)$) by some estimates $\hat \cD_\theta(0)$, and use this information to exploit the estimated optimal model
\begin{equation*} \textstyle
\hat \theta \in \argmin_{\theta}\big\{\widehat{\PR} (\theta) \triangleq \sum\nolimits\nolimits_{a \in \cA} \hat \cD_\theta(a)\Ex\big[\ell(\theta;Z)\mid A = a\big] \big\}.
\end{equation*}
We adopt a structure that alternates between estimating $\theta \mapsto \cD_{\theta}(0)$ and $\theta^{\star}$ sequentially improves the estimation of $\theta \mapsto \hat \cD_{\theta}(0)$ and $\hat \theta$. Define exponentially increasing intervals (called episodes) $\mathcal{J}_k$ for $k \in [K]$, such that $|\mathcal{J}_1|=\tau_o$ and $|\mathcal{J}_k|= \tau_o 2^{k-1}$ for $k=2,\dots, K$ so that $\oplus_{k=1}^K |\mathcal{J}_k|=M$, which means $K = \log_2(1+M/\tau_o)$. We divide every episode $\mathcal{J}_k$ into two sub-phases: the \textit{exploration} phase, with indexes $\mathcal{I}_k$ and an \textit{exploitation} phase, with indexes $\mathcal{I}'_k$. In the exploration phase, we essentially use Algorithm \ref{alg:seq-design-optial-ours}, that is we improve the estimate $\hat \cD_\theta(0)$ by updating $\hat \cD_\theta^{(k-1)}(0) \leftarrow \hat \cD_\theta^{(k)} (0)$, using optimal design models $\theta_{m}$ for $m \in \mathcal{I}_k$. In the exploitation phase, we constantly deploy
\begin{align}\label{eq:estimated-PR}
\hat \theta_k \in \argmin_{\theta}\Big\{\widehat{\PR}_k (\theta) \triangleq \sum\nolimits_{a \in \mathcal{A}} \hat \cD_\theta^{(k)} (a) \Ex[\ell(\theta;Z)|A=a]\Big\}.
\end{align}
We summarize our procedure in Algorithm \ref{alg:seq-design-doubling}.
\begin{algorithm}
\caption{Sequential Design with Doubling trick}\label{alg:seq-design-doubling}
\begin{algorithmic}[1]
\STATE Let $\mathcal{J}_1,\dots,\mathcal{J}_K$ sequential episodes with $\mathcal{J}_1 = \{1,\dots, \tau_o\}$, and $\mathcal{J}_k=\mathcal{I}_k \cup \mathcal{I}'_k$ for $k=2,\dots,K$, where $\mathcal{I}_k = \{\tau_o(2^{k-1} - 1)+1, \dots, a_k\}$ is the exploration index phase, where $a_k = (\tau_o2^{k-1})^{\alpha}$ for some $\alpha \in (0,1)$, and $\mathcal{I}'_k = \{a_k+1, \dots, \tau_o(2^{k} - 1)\}$ is the exploitation index phase.
\STATE For $k=1$ let $\hat d_1^*$ be the uniform density in $[0,1]$.
\FOR{$k=1,\dots K$}
\STATE For every $m \in \mathcal{I}_k$ draw $\iid$ samples $b_m$ from the estimated optimal design $\hat d_{k}^*$ and record $\hat \pi_m$ (see Remark \ref{remark:estimate-hatpi}).
\STATE Based on $\{\hat \pi_m\}_{m \in \mathcal{I}_k}$ update $\{\hat \cD_\theta^{(k)}(a);a\in \cA\}$, $\hat \sigma_k^2$ and the design density $\hat d_{k+1}^* \propto \hat \sigma_k$.
\STATE For every $m \in \mathcal{I}'_k$ deploy the same $\hat{\theta}_k = \argmax_{\theta} \widehat{\PR}_k(\theta)$, where $\widehat{\PR}_k$ is defined in \eqref{eq:estimated-PR}.
\ENDFOR
\end{algorithmic}
\end{algorithm}
To evaluate the goodness of Algorithm \ref{alg:seq-design-doubling} we define the total regret:
\begin{equation}\label{def:regret}
    \operatorname{Reg}(M) \triangleq \sum\nolimits_{k\in [K]}\sum\nolimits_{m \in \mathcal{J}_k} \Big[\PR(\theta^{\star}) -\widehat{\PR}(\theta_{m,k})\Big]
\end{equation}
which is a random quantity because $\theta_{m,k}$ depends on the data, and where
\begin{align}\label{eq:f_m,k}
\theta_{m,k} \text{ such that } b_m =b(\theta_{m,k}) \overset{\iid}{\sim} \hat{d}_k^* &\quad ,m \in \mathcal{I}_k \nonumber\\
\theta_{m,k} = \theta_{k} \in \argmin_{\theta}\widehat{\PR}_k(\theta) &\quad ,m \in \mathcal{I}'_k.
\end{align}
In the exploration phase ($\ie$ $\mathcal{I}_k$), we select models that improve the accuracy of the estimation of $\cD_\theta(0)$. The longer the length of the exploration phase, the smaller is $\|\cD_\theta(0)-\hat \cD_\theta(0)\|_{\infty} \triangleq \sup_{\theta}|\cD_\theta(0)-\hat \cD_\theta(0)|$, but the remaining exploitation phase ($\ie$ $\mathcal{I}_k'$) might be too short to guarantee a small regret. Similarly, if the exploration phase is short, $\hat \cD_\theta(0)$ will not be accurate enough to reduce the total regret. This suggests that there exists an optimal length for the exploration phase that guarantees minimal regret. For this reason in Algorithm \ref{alg:seq-design-doubling} we have defined a value $\alpha \in (0,1)$ and $a_k = |\mathcal{I}_k| = |\mathcal{J}_k|^{\alpha} = (\tau_o2^{k-1})^{\alpha}$, and we will show in Theorem \ref{thm:regret_bound} that there exists an optimal choice for such $\alpha$ that minimizes total regret, and $\alpha$ will depend on the convergence rate of $\|\cD_\theta(0)-\hat 
\cD_\theta(0)\|_{\infty}$. We assume that 
\begin{assumption}\label{assumption:regret}
$\Ex[\ell(f,X)|A=a]$ is uniformly bounded in $f$ and $a$. 
\end{assumption}

\begin{theorem}\label{thm:regret_bound}
Consider the definitions and procedure in Algorithm \ref{alg:seq-design-doubling}. Suppose that there exists some $\eta \in(0,1)$ such that, $\|\cD_\theta(0)-\hat \cD_\theta(0)\|_{\infty} = \mathcal{O}_P\left((\nicefrac{\log(|\mathcal{I}_k|)}{|\mathcal{I}_k|})^{\eta}\right)$ for each $k \in [K]$ and there exists $\delta \in (0,1)$ so that $\| \hat{d}^*_k - d^* \|_{\infty} = \mathcal{O}_P\left((\nicefrac{\log(|\mathcal{I}_k|)}{|\mathcal{I}_k|})^{\delta}\right)$. Under Assumptions \ref{assumption:regret}, the optimal value $\alpha$ that minimizes the total regret is $\alpha = 1/(1+\eta)$, which implies the following
\[
\begin{aligned}
    \operatorname{Reg}(M) = \mathcal{O}_P( M^{\nicefrac{1}{1+\eta}}\log^{\eta}(M)), \quad
    \operatorname{REL}(\hat{d}^*_K) = \mathcal{O}_P\left(M^{- \nicefrac{\delta}{1+\eta}}\log^{\delta}(M)\right) &\text{ as }M \rightarrow \infty.
\end{aligned}
\]
\end{theorem}

\begin{remark}
As we mentioned in Section \ref{sec:Sequential_method-doubling-trick}, if $\sigma(\cdot)$ is a continuous function of $F$ (see $\eg$ Example \ref{ex:CL-sequential-design}, where $\sigma^2\propto F\bar F$), then $\delta \equiv \eta$.
\end{remark}

\begin{remark}\label{remark:regret_bound}
For one-dimensional isotonic regression we have $\eta= \nicefrac{1}{3}$ (see Proposition \ref{thm:uniform_convergence}) that leads to regret of order $M^{\nicefrac{3}{4}}$. For other non-parametric estimates, such as kernel, splines, see \eg\  \citep[Section  3]{zhao2012sequential}, $\eta=\nicefrac{\beta}{2\beta + 1}$ where $\beta \triangleq \max\{\gamma\in \bN :\sF_0 \text{is $\gamma$ times continuously differentiable}\}$, leading to regret of order $M^{\nicefrac{2\beta+1}{3\beta + 1}}$.
\end{remark}

We compare our Theorem \ref{thm:regret_bound}, with the result provided by \cite{jagadeesan2022Regret}. The main difference is that, while we estimate $\PR$ by plugging in an estimate of the distribution shift, they sample from the distribution shift to estimate $\PR$. In Theorem 4.2 they get a regret bound of the order $\mathcal{O}(M^{\nicefrac{d+1}{d+2}})$. However, as mentioned in Remark \ref{remark:regret_bound}, we can achieve $\operatorname{Reg}(M)=\widetilde{\mathcal{O}}_P(M^{\nicefrac{2\beta+1}{3\beta+1}})$. Our regret bound is lower than $\operatorname{Reg}_{\textit{mean}}(M)$ (excluding $\log(M)$ factors) for $\beta \geq 1$ and $d\geq 2$, we defer to Appendix \ref{sec:regret_comparison}.
